Interacting Safely with an Unsafe Environment

We give a presentation of Pure type systems where contexts need not be well-formed and show that this presentation is equivalent to the usual one. The main motivation for this presentation is that, when we extend Pure type systems with computation rules, like in the logical framework Dedukti, we want to declare the constants before the computation rules that are needed to check the well-typedness of their type.

==> eptcsdata.tex <==
\providecommand{\firstpage}{30}
\providecommand{\publicationstatus}{E. Pimentel and E. Tassi (Eds.): Logical Frameworks\\ and Meta-Languages: Theory and Practice (LFMTP 2021)\\
EPTCS 337, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.337.3}{10.4204/EPTCS.337.3}}

